On Data-Selective Learning

Adaptive filters are applied in several electronic and communication devices like smartphones, advanced headphones, DSP chips, smart antenna, and teleconference systems. Also, they have application in many areas such as system identification, channel equalization, noise reduction, echo cancellation, interference cancellation, signal prediction, and stock market. Therefore, reducing the energy consumption of the adaptive filtering algorithms has great importance, particularly in green technologies and in devices using battery. In this thesis, data-selective adaptive filters, in particular the set-membership (SM) adaptive filters, are the tools to reach the goal. There are well known SM adaptive filters in literature. This work introduces new algorithms based on the classical ones in order to improve their performances and reduce the number of required arithmetic operations at the same time. Therefore, firstly, we analyze the robustness of the classical SM adaptive filtering algorithms. Secondly, we extend the SM technique to trinion and quaternion systems. Thirdly, by combining SM filtering and partial-updating, we introduce a new improved set-membership affine projection algorithm with constrained step size to improve its stability behavior. Fourthly, we propose some new least-mean-square (LMS) based and recursive least-squares based adaptive filtering algorithms with low computational complexity for sparse systems. Finally, we derive some feature LMS algorithms to exploit the hidden sparsity in the parameters.

==> Abbreviations.tex <==
\chapter*{Abbreviations}

==> abbre.tex <==
\chapter*{List of Abbreviations}
 

\begin{table}[t!]
\begin{tabular}{lll}
AP & & Affine Projection\\
AR & & Auto Regressive\\
LMS & & Least-Mean-Square\\
MSE & & Mean-Squared Error\\
NLMS & & Normalized LMS\\
PAPA & & Proportionate AP Algorithm\\
SM-AP & & Set-Membership Affine Projection\\
SM-NLMS & & Set-Membership Normalized LMS\\
SM-PAPA & & Set-Membership PAPA\\
SSM-AP & & Sparsity-aware SM-AP
\end{tabular}
\end{table}

==> appenA.tex <==
\chapter{}

